COMPARE: Accelerating Groupwise Comparison in Relational Databases for Data Analytics

Data analysis often involves comparing subsets of data across many dimensions for finding unusual trends and patterns. While the comparison between subsets of data can be expressed using SQL, they tend to be complex to write, and suffer from poor performance over large and high-dimensional datasets. In this paper, we propose a new logical operator COMPARE for relational databases that concisely captures the enumeration and comparison between subsets of data and greatly simplifies the expressing of a large class of comparative queries. We extend the database engine with optimization techniques that exploit the semantics of COMPARE to significantly improve the performance of such queries. We have implemented these extensions inside Microsoft SQL Server, a commercial DBMS engine. Our extensive evaluation on synthetic and real-world datasets shows that COMPARE results in a significant speedup over existing approaches, including physical plans generated by today's database systems, user-defined function (UDF), as well as middleware solutions that compare subsets outside the databases.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
Comparing and finding related entities is a common operation in  data analytics~\cite{bohm2004k,agrawal1993efficient,lin1995fast} and visual analytics applications~\cite{zenvisagevldb,ding2019quickinsights,macke2018adaptive,seedb}.
 For example, a market analyst may be interested in finding products whose sales over time are comparable to that of a best selling product, a financial analyst may look for stocks with similar prices to that of a given stock (Figure ~\ref{fig:tableaudash}), and a real estate agent may want to identify cities with matching house prices to that of a specific city
 (Figure~\ref{fig:zenvisagedash}). 
 As depicted in Figure~\ref{fig:comaparemechanics}, in all these examples,  each entity (e.g., product, stock, house) is  represented via a {\em group of tuples} in a relational database, and finding related entities corresponds to searching for related groups of tuples.
 % often compared using distance measures such as Euclidean distance or other $L_p$ norms measures~\cite{agrawal1993efficient,zenvisagevldb}.

In order to support such use-cases, it is crucial for a database query language to be able to {\em succinctly} express  and {\em efficiently} execute  comparative queries. Unfortunately, as we describe shortly, the standard SQL (SQL:2016) does not allow a concise specification of comparison between groups of tuples---often requiring expensive  joins and sub-queries even for conceptually simple comparative queries. 
%As a result, it is extremely difficult to write, understand, and maintain such queries.
Furthermore, the complexity of query specification makes it hard for query optimizers to identify efficient algorithms to evaluate such queries. 

To illustrate, we consider the following  example of an analytic query.


%number of conceptually simple comparative queries involving 
\eat{
, and for query processing engine to be able to {\em efficiently} evaluate such queries.
Second, it is very difficult for
a query optimizer to identify efficient algorithms.

A number of distance measures such as Euclidean distance, Mahalanobis, and Manhattan


 many nearest neighbor-based algorithms use  Euclidean, Mahalanobis, and Manhattan distance measure to compare between two groups of tuples as one of the most critical computations involved in attaining the objective.  

Many nearest neighbor algorithms use  distance measures such as Euclidean, Mahalanobis, and Manhattan
to compare between 

 distance measure to compare between two groups of tuples as one of the most critical computations involved in attaining the objective


 groups of tuples is a common operation during data exploration~\cite{wongsuphasawat2017voyager, ding2019quickinsights,lee2019you, seedb-tr,zenvisagevldb,wongsuphasawat2017voyager,macke2018adaptive}. For example, many nearest neighbor-based algorithms use  Euclidean, Mahalanobis, and Manhattan distance measure to compare between two groups of tuples as one of the most critical computations involved in attaining the objective.  Similarly, visualization tools support expression languages (e.g., Data Analysis Expressions (DAX) in PowerBI~\cite{powerbidax}, Level of Detail (LOD) expressions in Tableau~\cite{tableaulod}, ZQL in Zenvisage~\cite{zenvisagevldb}) let users select one or more visualizations of their interest, and automatically show the related visualizations. For instance, Figure~\ref{fig:tableaudash} depicts a Tableau dashboard where a market analyst selects the visualization of Boeing stock price to visualize other companies with similar stock trends over time. As another example, Figure~\ref{fig:zenvisagedash} depicts a dashboard in Zenvisage, where a real estate analyst can either drag or drop the visualization of a specific state, or write a query in a table to find other states with similar housing price trends. 


In order to support such applications, it is crucial for a database query language to be able to {\em succinctly} express common comparative queries, and for query processing engine to be able to {\em efficiently} evaluate such queries. Unfortunately, the standard SQL (SQL92) does not allow the concise expression of a number of conceptually simple queries involving comparison between two groups of tuples, requiring additional joins and subqueries with a high degree of redundancy. There
are two important consequences of such redundancy.
First, it is very difficult to write, understand, and
maintain such queries. Second, it is very difficult for
a query optimizer to identify efficient algorithms.
}

\begin{figure}	
	\begin{subfigure}{0.55\columnwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/sqlquery.pdf}}}}
		
		\caption{\smallcaption{ SQL Query for Example 1} }
		\label{fig:querymotiv}
	\end{subfigure}
	\hspace{-0.6cm}
	\begin{subfigure}{.50\columnwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/queryplan.pdf}}}}
		\caption{\smallcaption{Query Plan}}
		\label{fig:planmotiv}
	\end{subfigure}
	\caption{ \smallcaption{The SQL Query and the query plan for Example 1 for finding 10 products where the average minimum difference of sales to that of product `Inspiron' is smallest} 
	 }
	\vspace{-5pt}
	\label{fig:productresults}	
\end{figure} 

\stitle{Example 1.} A market analyst notices that the sales of Inspiron over weeks have been increasing (depicted by a green line chart in Figure~\ref{fig:motiv}c) despite the drop in the sales of most of the other products. She is therefore interested in finding another product 
 whose sum of squared differences in sales to that of  inspiron in minimum. The comparison metric---sum of squared differences or squared Euclidean distance, is often used for comparing two trends~\cite{rss}. For instance, in Figure~\ref{fig:motiv}c, the sales trend of XPS13 (blue line chart) look similar to that of Inspiron, and  has the minimum sum of squared differences to that Inspiron.
 


Figure~\ref{fig:querymotiv} depicts the SQL query for the above example, and is arguably  the most efficient way of writing this query in \db\footnote{A commercial DBMS --- anonymized for double-blind reasons.} with standard relational operators such as scan, join, aggregation, filters, and window analytics function such as rank.  Figure~\ref{fig:planmotiv} depicts a simplified version of the query plan generated by \db for this SQL  query.  At a high level, the query first creates an intermediate relation via a self-join between the tuples of product Inspiron and the rest of the products (highlighted in red). Next, a sequence of scalar operations and aggregations  are performed on the intermediate relation to compute the similarity (i.e., sum of squared differences) score of each product with Inspiron. Finally, a filter followed by a join operation output the tuples of $10$ products with minimum scores. As we can see, this query is quite complex, requiring three sub-queries, two joins, and two scans, making it difficult for data analysts to express such queries.


\begin{figure*}	
	\vspace{-20pt}
	\hspace{-0.2cm}
	\begin{subfigure}{0.38\textwidth}
		\vspace{-5pt}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/tableau-snapshot.pdf}}}}
		\caption{\smallcaption{Stock similarity search		in Tableau~\cite{tableau}}}
		\label{fig:tableaudash}
	\end{subfigure}
	\hspace{0.2cm}
	\begin{subfigure}{.375\textwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/zenvisage-snapshot.pdf}}}}	
		\caption{\smallcaption{Searching states with comparable housing price trends in Zenvisage~\cite{zenvisagevldb} }}
		\label{fig:zenvisagedash}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.20\textwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/motivation4.pdf}}}}
		\caption{\smallcaption{Mechanics of a \\ Comparative Query \fixlater{fix}}}
		\label{fig:comaparemechanics}
	\end{subfigure}
	\vspace{-10pt}
	\caption{ \smallcaption{(a) and (b) depict comparative queries in Tableau and Zenvisage, and (c) depicts the mechanics of a comparative query.} }
	\label{fig:motiv}	
	\vspace{-5pt}
\end{figure*} 



Even when such a query is machine generated, the complexity often results in poor performance as it is difficult to capture the semantics of \emph{groupwise tuple comparisons} between the entities using existing operations. For instance, the input to self-join in the above example consists of two groups of tuples: one for Inspiron and one for the rest of the products, with the join comparing all pairs of tuples between the two groups. In contrast, if we treat each  product as an independent group, sort them by week, and join each separately with Inspiron---we can avoid all-pairs comparison, and  reduce the number of tuple comparisons drastically by a factor equal to the number of products. Furthermore, while we only need the  aggregated result for each group, i.e., the sum of squared differences with respect to the tuples of Inspiron (reference group), the join generates large  intermediate results---one tuple for each pair of matching tuples between the reference group and other groups. The intermediate results is often materialized by subsequent operations (e.g., sort, aggregation) resulting in a substantial overhead.

\eat{
For instance, the self-join results in generation of large intermediate data, i.e., one tuple for each pair of matched tuples between the reference group and other groups, which are further materialized by subsequent operations (e.g., sort, aggregates) resulting in a substantial overhead.  Furthermore, the self-join does not  capture the semantics of group-wise comparison between tuples of products. Instead, the execution of self-join involves costly all-pairs comparisons between the tuples of the reference product and the rest of the products, resulting in large number of tuple comparisons( proportional to the product of the size of the reference product and  the size of all other products).
}



%However, the existing query execution strategy of execution of join is agnostic of the scalar or aggregate  expressions applied on the join output, thereby missing optimizations that can potentially reduce the number of tuple comparisons during join. 

The semantic properties of comparison metric (e.g., sum of squared differences) can often be used to reduce the number of comparisons between groups of tuples. To illustrate, consider a simple query that finds the \amax \xspace difference in the sales of two products.  Here, comparing only the tuples with smallest and largest values of sales for each product is sufficient. Unfortunately, the existing approach is to first perform a cross join for computing differences between all pairs of tuples, followed by an aggregation to find the \amax \xspace difference. Thus, the existing techniques do not take advantage of the properties of the aggregation functions.


\fixlater{can we give related references}

%Finally, as part of large data analytics pipelines~\cite{abuzaid2018diff}, a comparative operation can  occur as a sub-operation within a larger SQL query, with arbitrary joins as its input, and other operators consuming its output.  In those cases, we would ideally like the query optimizer to find a plan that is optimal for the entire query. Unfortunately, given the complexity of a comparative query, we observe that query optimizers are unable to apply even standard optimizations. Moreover, in certain cases such as PK-FK join, and aggregate queries, push-down and pull-up transformations can be applied to generate more efficient plans.



 
 
 %For instance, for query 2, the self-join results in  $99 \times 10^6$ tuples since every tuple in  product 'Inspiron' is matched with every tuple of other products. The intermediate tuples are further materialized by subsequent operations (e.g., sort, aggregates) resulting in a substantial overhead. However, many comparison criteria, e.g., $L_p$ norms, involve simple aggregates (\aavg, \asum, \amin, \amax) and scalar operations such as differences, and thus comparison results can be computed efficiently in an incremental fashion (much like simple aggregates), without generating or materializing  intermediate tuples. 


%To the best of our knowledge, both Figure~\ref{fig:querymotiv} and Figure~\ref{fig:planmotiv} are representative of how other relational databases will also express and execute queries such as query $1$, and are arguably the most optimal way of executing query $1$ with standard relational operators such as scan, join, aggregation, filters, and window analytics function such as rank.While it is difficult for data analysts to directly write such a query, even when it is automatically generated, the complexity results in  long execution times because of the missed optimization opportunities that we discuss next.





%While it is difficult for data analysts to directly write such a query, even when it is automatically generated, the complexity results in  long execution times because of the missed optimization opportunities. For example, the self-join results in generation of large intermediate data, i.e., one tuple for each pair of matched tuples between the reference group and other groups, which can be avoided without affecting the end results. For instance, for query 2, the self-join results in  $99 \times 10^6$ tuples since every tuple in  product 'Inspiron' is matched with every tuple of other products. The intermediate tuples are further materialized by subsequent operations (e.g., sort, aggregates) resulting in a substantial overhead. However, many comparison criteria, e.g., $L_p$ norms, involve simple aggregates (\aavg, \asum, \amin, \amax) and scalar operations such as differences, and thus comparison results can be computed efficiently in an incremental fashion (much like simple aggregates), without generating or materializing  intermediate tuples. 


%The self-join essentially performs all-pairs comparisons between the tuples of the reference group and the rest of the groups, with the overall number of comparisons proportional to product of the size of the reference group and  the size of all other groups. For example, if there are $100$ products, each consisting of $10^3$ tuples, the self-join in query $1$ performs a total of $10^3 \times 99 \times 10^3$ tuple comparisons. However, in many cases, all pairs comparisons can be avoided by performing \emph{groupwise comparisons, i.e., comparing each group independently with the reference group}. For example, for query 1, sorting tuples of each product on week and then comparing them independently reduces the number of comparisons by a factor of $10^3$ (i.e, the the size of each group), and is extremely parallelizable --- both leading to massive speed-up in performance. Unfortunately, the self-joins in relational databases do not support the notion of \emph{group-wise comparisons},  thereby missing potential optimizations.

%Relational databases typically do not optimize for join and aggregation operations based on the scalar or aggregate  expressions that are computed on their output, missing key potential optimizations that can further reduce the number of tuple comparisons and runtimes of comparative queries. For example, consider a simple query where we want to find the \amax \xspace difference in the sales of two products.  Here, comparing only the tuples with smallest and largest values of sales for each product is sufficient. Unfortunately, the existing SQL execution performs a cross join, computing differences between all pairs of tuples from the  products, followed by an aggregation to find the \amax \xspace difference.

%Finally, a comparative query can occur as a sub-query within a larger SQL query, with arbitrary relational expression such as joins as its input, and other operators consuming its output.  In those cases, we would ideally like the query optimizer to find a plan that is optimal for the entire query. Unfortunately, given the complexity of a comparative query, we observe that query optimizers are unable to apply even standard optimizations. Moreover, in certain cases such as PK-FK join, and aggregate queries, push-down and pull-up transformations can be applied to generate more efficient plans.



\stitle{Our Solution.} 
In this paper, we take an important step towards making specification of the comparison queries easier as well as ensuring efficient processing of such queries. To do so,  we introduce
both a logical operator and a physical operator in relational databases relational databases, as described below.

\stitle{C1. Groupwise comparison as a first class construct (Section~\ref{sec:compareoverview})}. While prior work have proposed extensions~\cite{chatziantoniou1996querying,chatziantoniou2007using,gray1997data,cunningham2004pivot,tang2015similarity} for succinctly writing complex group-by aggregate queries, expressing comparison between groups of tuples remains a challenge. Therefore, we introduce a new logical operation, \optr ($\Phi$), as a first class  relational construct, and formalize its semantics that help capture a large class of frequently used comparative queries.  While \optr does not give additional expressive power to the relational algebra, it
reduces the complexity of specifying comparative queries and facilitates 
optimizations that are otherwise missed by the query optimizer and the execution engine. We also propose extensions to SQL syntax
that allows intuitive and more concise specification of comparative queries.

%While it is also possible to extend the optimizer with algebraic transformation rules to translate comparative sub-queries expressed using standard SQL operators to $\Phi$.

%While \optr does not add to the expressivity of relational algebra,  it helps introduce the notion of subset comparison in the optimizer, making it easier to represent and reason about optimizations, as well as more effectively inter-operate with other relational operators.
\fixlater{motivate the need for complex query?}

\stitle{C2. Efficient processing via new physical operator (Section~\ref{sec:phyop})}. 
%One option to execute \optr operation is to use user-defined functions (UDFs). However, UDFs have limited interoperability with other operators, and are less amenable to logical optimizations. 
We introduce a new physical operator, $\Phi_P$, for the logical operator \optr, that ensures  efficient execution of comparative queries. $\Phi_P$ exploits the semantics of \optr operation to partition and compare tuples in a groupwise manner that significantly reduces the number of tuple comparisons as well as the size of intermediate data.  In addition, $\Phi_P$ incorporates several  physical optimizations that prune a large number of tuple comparisons without affecting the accuracy.
\eat{
	For instance, for the example 1, $\Phi_P$ minimizes tuple comparisons and intermediate data by partitioning the input relation and performing comparison independently and in parallel for each product. In addition, $\Phi_P$ applies several physical optimizations that help in identifying the top $K$ products without computing the exact score. At a high-level, $\Phi_P$ can prune low scoring products without performing tuple-level comparisons by only comparing a few coarse-grained aggregates of partitions, that are faster to compute. Among the partitions that are not pruned, $\Phi_P$ further prioritizes tuple comparisons in an order that leads to faster convergence of the top $K$ partitions.
}
%For example, $\Phi_P$ summarizes sales of each product using coarse-grained aggregates that help prune out low scoring product without performing their tuple-level comparisons. $\Phi_P$ further prioritizes products that are most likely to be in top K and performs tuple comparison in an order that minimize wastage of tuple comparisons. 

\stitle{C3. Optimizer integration using new transformation rules (Section~\ref{sec:optint})}. 
We introduce new  algebraic transformation rules that allows the query optimizer to transform the logical tree containing the COMPARE operator into equivalent logical trees that may be more efficient. These include pushing COMPARE below join, pushing aggregates below COMPARE, and enable translation from logical ($\Phi$)  to physical ($\Phi_p$).
We also introduce a cost model for the physical operator $\Phi_p$ that enables the optimizer to cost plans containing $\Phi_p$. 

%We integrate \optr within the optimizer of \db that enables automatic translation from logical ($\Phi$)  to physical ($\Phi_p$) operator using cost-based optimization.  We further extend the optimizer with algebraic transformation rules that allow logical optimizations when \optr occurs as a sub-query in a larger SQL query. 

% of queries where \optr occurs as a sub-component in a larger query. via reordering of \optr to minimize the overall query processing time of queries where \optr occurs as a sub-component in a larger query. 
\stitle{C4. Extensions (Section~\ref{sec:extensions}).}  
We  discuss several important  extensions that build on the core ideas of \optr. For example, we show how to use multiple groups as references for comparison, how we can support query-by-sketch systems~\cite{visual2, timesearcher,zenvisagevldb,lee2019you}, and how we can support additional comparison metrics and user-defined functions (UDF).


\stitle{C5. Implementation and evaluation (Section~\ref{sec:exp}).}  We have prototyped our techniques in \db engine, including the logical operator \optr and the new physical operator $\Phi_p$. We perform a thorough performance study of the extended \db with that of the unmodified \db on both real world and synthetic datasets. We also varied the characteristics of comparative queries to test the performance and scalability of optimizations. Our experiments demonstrate that introducing \optr results in an improvement in performance ranging from $3$$\times$ to $60$$\times$.




\eat{
%In summary, while \optr does not give additional expressive power to the relational algebra, it makes comparative queries much easier to write, and allows efficient processing via logical and physical optimizations that are difficult to apply with existing operators. In  rest of the paper, we describe each of the above contributions in detail.







\stitle{P3. Large intermediate data.} 
The self-join results in generation of large intermediate data, i.e., one tuple for each pair of matched tuples between the reference group and other groups, which can be avoided without affecting the end results. For instance, for query 2, the self-join results in  $99 \times 10^6$ tuples since every tuple in  product 'Inspiron' is matched with every tuple of other products. The intermediate tuples are further materialized by subsequent operations (e.g., sort, aggregates) resulting in a substantial overhead. However, many comparison criteria, e.g., $L_p$ norms, involve simple aggregates (\aavg, \asum, \amin, \amax) and scalar operations such as differences, and thus comparison results can be computed efficiently in an incremental fashion (much like simple aggregates), without generating or materializing  intermediate tuples. 


\eat{
	\stitle{Problem 3. Large intermediate size.} The existing approach creates new tuples by joining all pairs of tuples between subsets that are compared. For example, if the number of 
	tuples for each product is $100$ and the number of products is $50$, the size of the intermediate table is $50.100^2$ times the original size of the relation. More specifically, the size of the intermediate relation is proportional to the number of tuples that are compared.
	The cost of performing a join to generate such large intermediate relations and performing subsequent operations (e.g., aggregation) that often require materialization (e.g, for sorting) is substantial. 
}

\stitle{P4. Comparison criteria agnostic.} Relational databases typically do not optimize for join and aggregation operations based on the scalar or aggregate  expressions that are computed on their output, missing key potential optimizations that can further reduce the number of tuple comparisons and runtimes of comparative queries. For example, consider a simple query where we want to find the \amax difference in the sales of two products.  Here, comparing only the tuples with smallest and largest values of sales for each product is sufficient. Unfortunately, the existing SQL execution performs a cross join, computing differences between all pairs of tuples from the  products, followed by an aggregation to find the \amax \xspace difference.

\stitle{P5. Missed inter-operator optimizations.} Finally, a comparative query can occur as a sub-query within a larger SQL query, with arbitrary relational expression such as joins as its input, and other operators consuming its output.  In those cases, we would ideally like the query optimizer to find a plan that is optimal for the entire query. Unfortunately, given the complexity of a comparative query, we observe that query optimizers are unable to apply even standard optimizations. Moreover, in certain cases such as PK-FK join, and aggregate queries, push-down and pull-up transformations can be applied to generate more efficient plans.


%pushed down below operators, or other operators such as filters and aggregates can be pushed down below a comparative quer
%and output the relation over which a comparative query can be expressed can be any arbitrary relational expression, involving multiple joins





%Because of the complex combination of multiple logical operator as depicted in the above query plan, the notion of comparison between subset of tuples is not straightforward to dissect. Moreover, existing optimizers analyze the properties (e.g., sorting, grouping, selectivity) on a per operator basis to select various logical optimizations such as below join push-down and predicate push-down. Unfortunately, we observe that the optimizers are unable to apply such optimizations for the entire sub-tree of logical operators.



\eat{
	
	\stitle{Motivating Example.} Anna, an infrastructure support analyst, notices unexpected changes in the cpu usage for $2$ machines, $M_1$ and $M_2$, over the past week as depicted in Figure~\ref{fig:relationmotiv}. For troubleshooting, she wants to understand whether there are additional machines with similar cpu usage profiles. The most commonly used metrics for comparing trends are $L_p$ norms such as Euclidean distance or sum of differences. If trends do not align point-wise over time, another option is to use \emph{min-max} aggregation, to find machines where maximum cpu usage differences with those of $M1$ or $M2$ between any two time point is minimum, or search for ones where the average difference in cpu across all points is minimum. Nevertheless, all these comparison functions are examples of aggregated distance functions, involving simple aggregations (e.g., $sum, avg, min, max$) over functions of differences. We list the three potential queries  using these comparison functions below.
	
	\emph{$Q1$. Visualize 10 machines that have smallest sum of differences in the cpu usage trends over hours with respect to those of $M_1$ and $M_2$.
	} 
	
	\emph{$Q2:$ Visualize $10$ machines whose maximum differences in CPU usages with those of $M1$ and $M2$ at any point during the week were smallest.}
	
	\emph{$Q3:$ Visualize $10$ machines whose average differences in the CPU usage with those of $M1$ and $M2$ across all points were smallest.}
	
	There are multiple ways to issue the above queries. The simplest option is to generate a large collection of visualizations, one for each machine and manually step through them to find the ones that have similar behaviour. Unfortunately, the process of manual examination is not scalable to $10$s of $1000$s of machines. Therefore, a better option is to either directly write a SQL query or use visual analytic tools that support high level language for expressing comparison among visualizations and automatically transform them to SQL queries. (e.g., Tableau's Level of Detail Expression, PowerBI's PowerQuery, Zenvisage, SeeDB).
	
	\stitle{ Existing query execution strategy.} 
	%While these queries differ in their comparison function, they all involve comparison between tuples across pairs of subsets of tuples. 
	Figure~\ref{fig:queryplanmotiv} depicts a simplified version of the query plan generated by RDBMS for executing SQL versions of above queries, and consists of five steps: (i) a filter to select $2$ subsets of tuples  (one each for $M_1$ and $M_2$), where a tuple records the CPU usage at a specific hour, (ii) a join between the tuples of the entire relation and reference subsets, generating an intermediate relation, (iii) a sequence of scalar operations and aggregations  to compute the aggregated distance ($score$) for every other machine, (iv) a filter to select the names of  $10$ machines with minimum scores, and finally (v) another join to select and output the subset of rows correspond to top $10$ machines. There are four  key problems with this execution strategy. 
	
	
	
	
	\eat{
		\begin{figure}
			\centerline {
				\hbox{\resizebox{.83\columnwidth}{!}{\includegraphics{./figs/queryplan.pdf}}}}
			\vspace{-10.5pt}
			\caption{\smallcaption{An example of a query plan produced by existing query optimizers for comparative queries in the motivating example.}}
			\label{fig:queryplanmotiv}
			\vspace{-10.5pt}
		\end{figure}
	}
	
	\eat{
		\begin{figure*}
			\centerline {
				\hbox{\resizebox{\textwidth}{!}{\includegraphics{./figs/diag1.pdf}}}}
			\vspace{-10.5pt}
			\caption{\smallcaption{Impact of the segment size on segment-aggregates based pruning $Q_1$}}
			\label{fig:varysegmentq1}
			\vspace{-2.5pt}
		\end{figure*}
	}
	
	\eat{
		\begin{figure}
			\centerline {
				\hbox{\resizebox{0.55\columnwidth}{!}{\includegraphics{./figs/queryplan2.pdf}}}}
			\caption{\smallcaption{An example query plan produced by optimizers for comparative queries}}
			\label{fig:queryplanmotiv}
			\vspace{-15.5pt}
		\end{figure}
	}
	
	\stitle{(1) Complex with redundant scan and join.} As depicted in the above query plan, expressing comparison between groups (or subsets) of tuples requires complex and redundant combination of multiple operations such as scans and joins. The is primarily because there is not direct mechanism for comparing groups (or subsets) of tuples in relational algebra, and it is extremely hard for an optimizer to dissect the notion of group-wise comparison abstracted across several operators in this plan. Moreover, there are no physical operators that support efficient algorithms for such operations. Finally, it is extremely hard to write, understand, and maintain such queries.
	
	
	\stitle{(2) Large intermediate size.} The existing approach creates new tuples by joining all pairs of tuples from subsets that are compared. For the above example involving two reference subsets and considering there are at least $100$ tuples for each machine, we see that the size of intermediate table for $Q_1$ is $2x$ more than the initial size, and for queries $Q_2$ and $Q_3$, the size is prohibitively large --- $100X$ the original size. Clearly, the cost of generating such large intermediate relations and performing subsequent operations (e.g., aggregation) on them is substantial. 
	
	
	\stitle{(3) Comparison agnostic.}  Comparison among subsets is typically done using aggregated distance functions as listed earlier, involving aggregation and scalar functions already supported in SQL. However, the existing execution approach is agnostic of  these functions, missing potential optimizations. As an extreme example, for finding maximum difference between two subsets, it is sufficient to to look at the differences among the tuples with maximum and minimum values. Unfortunately, the existing approach computes all differences between all pairs of tuples across the subsets, only to take the maximum; thereby wasting most of the effort.
	
	\stitle{(4) Missed inter-operator optimizations.} The optimzers leverage interesting properties to decide efficient plans that share grouping and sorting operations across operators. However, it is difficult to reason about such properties for a sub-graph of operators together. Similarly, it is difficult to apply logical optimizations such as join push-down and predicate push-down over the entire sub-graph.
	
}

\stitle{Our approach.} Our goal is to address the above limitations by reducing the complexity of query specification, and facilitating efficient processing of comparative queries. To do so,  we introduce both logical and physical extensions to relational databases, as described below.

\stitle{C1. Comparison as a first class construct (Section~\ref{sec:compareoverview})}. We introduce a new logical operation, \optr ($\Phi$), as a first class construct within the relational databases, and formalize its semantics that help capture a large class of frequently used comparative queries.  While \optr does not give additional expressive power to the relational algebra, it
reduces the complexity of specifying comparative queries and facilitates 
optimizations that are otherwise missed by the 
optimizer and the execution engine. We also propose extensions to SQL syntax
that allows intuitive and more concise specification of comparative queries.
%While it is also possible to extend the optimizer with algebraic transformation rules to translate comparative sub-queries expressed using standard SQL operators to $\Phi$.

%While \optr does not add to the expressivity of relational algebra,  it helps introduce the notion of subset comparison in the optimizer, making it easier to represent and reason about optimizations, as well as more effectively inter-operate with other relational operators.

\stitle{C2. Efficient processing via new physical operator (Section~\ref{sec:phyop})}. One option to execute \optr operation is to use user-defined functions (UDFs). However, UDFs have limited interoperability with other operators, and are less amenable to logical optimizations. We, therefore, introduce a new physical operator, $\Phi_P$, for the logical operator $\Phi$, that ensures  efficient execution of comparative queries. $\Phi_P$ exploits the semantics of \optr operation to partition and compare tuples in a manner that significantly reduces the number of tuple comparisons as well as the size of intermediate data.  In addition, $\Phi_P$ incorporates a number of physical optimizations that help avoid out many tuple comparisons for a large class of frequently used comparison functions without computing the exact results of groups.

\eat{
	For instance, for the example 1, $\Phi_P$ minimizes tuple comparisons and intermediate data by partitioning the input relation and performing comparison independently and in parallel for each product. In addition, $\Phi_P$ applies several physical optimizations that help in identifying the top $K$ products without computing the exact score. At a high-level, $\Phi_P$ can prune low scoring products without performing tuple-level comparisons by only comparing a few coarse-grained aggregates of partitions, that are faster to compute. Among the partitions that are not pruned, $\Phi_P$ further prioritizes tuple comparisons in an order that leads to faster convergence of the top $K$ partitions.
}
%For example, $\Phi_P$ summarizes sales of each product using coarse-grained aggregates that help prune out low scoring product without performing their tuple-level comparisons. $\Phi_P$ further prioritizes products that are most likely to be in top K and performs tuple comparison in an order that minimize wastage of tuple comparisons. 

\stitle{C3. Optimizer integration and logical optimizations (Section~\ref{sec:optint})}. 
We integrate \optr within the optimizer that enables automatic translation from logical ($\Phi$)  to physical ($\Phi_p$) operator using cost-based optimization.  We further extend the optimizer with algebraic transformation rules that allow logical optimizations when \optr occurs as a sub-query in a larger SQL query. 

% of queries where \optr occurs as a sub-component in a larger query. via reordering of \optr to minimize the overall query processing time of queries where \optr occurs as a sub-component in a larger query. 
\stitle{C4. Extensions (Section~\ref{sec:extensions}).}  
We  discuss four key extensions that build on the core ideas of \optr, including using multiple groups as references for comparison, supporting query-by-sketch systems~\cite{visual2, timesearcher,zenvisagevldb,lee2019you} where a sketch of the desired trend can be used as reference for finding similar groups, supporting user-defined functions (UDF), and handling missing values.


\stitle{C5. Implementation and evaluation (Section~\ref{sec:exp}).}  We have prototyped our techniques in  \db engine, including both the logical and physical operators. We perform a thorough performance comparison of the extended \db with that of the unmodified \db on both real world and synthetic datasets. We also varied the characteristics of comparative queries to test the effectiveness and scalability of physical and logical optimizations. Overall, our experiments demonstrate that introducing \optr results in an improvement ranging from $3$$\times$ to $60$$\times$.

In  the rest of the paper, we describe each of the above contributions in detail.

%In summary, while \optr does not give additional expressive power to the relational algebra, it makes comparative queries much easier to write, and allows efficient processing via logical and physical optimizations that are difficult to apply with existing operators. In  rest of the paper, we describe each of the above contributions in detail.


 


%In addition, it is also common for data analysts to directly issue custom SQL queries via connectors~\cite{customsql} supported in visualization tools, as well as using interactive data analytics IDEs such as SQL editors~\cite{sqleditor} and Jupyter notebooks~\cite{d2018aida,sqljupyter} for exploring visualizations.



The comparison computation involves computing simple arithmetic operations such as subtraction among
two or more matrices. 


Visualization tools support expression or formula languages (e.g., Data Analysis Expressions (DAX) in PowerBI~\cite{powerbidax}, Level of Detail (LOD) expressions in Tableau~\cite{tableaulod}, ZQL in Zenvisage~\cite{zenvisagevldb}) that facilitate specification of comparison criteria using simple aggregates (e.g. \asum, \aavg, \amin, \amax),  and scalar functions. 

Internally, the queries are translated into one or more SQL queries for performing computations inside the databases, that helps avoid large data transfer delays, as well as serialization and deserialization overheads between the client and databases. I

Unfortunately, the impedance mismatch between the operators in databases and the comparative analytical queries result in complex and inefficient SQL queries that hinder the performance of such queries, in some cases resulting in worse performance than their counterparts doing processing outside the databases. Therefore, in this work, our goal is to address this impedance mismatch for efficiently executing comparative queries inside the databases. We first give a few motivating examples, and describe the key limitations of existing SQL execution of comparative queries.


 
The distance computation involves computing simple arithmetic operations such as multiplication, subtraction among
 two or more matrices. 
 

The distance computation involves computing arithmetic operations such as multiplication, subtraction among
two or more matrices. Using a high level language to
compute these matrix computations may require the matrices to be held in memory, for larger matrices the program should some complex matrix transfers to and from
disk. There many types of distances used in machine learning algorithms such as Euclidean, Mahalanobis, Manhattan
etc which involve quadratic matrix computations. We use
Euclidean distance here to demonstrate the distance computation as it is popular and the other distances are generalizations of the Euclidean distance. The applications of
the Euclidean distance in machine learning algorithms for
performance purposes is demonstrated using clustering and
classification. K-Means [1, 6, 13], is one of the most popular clustering algorithms used widely due to its robustness,
convergence and it applies Euclidean distance to compute
the clusters. We use K-Means clustering and a Bayesian
classification based on K-Means to demonstrate the computation of Euclidean distance


Previous work has concentrated on the use of spatial
databases or stand-alone systems.
In these solution methodologies, changes to the database engine maybe necessary; for
example, new index structures or novel algorithms need to
be incorporated into the engine. This requirement poses a
limitation when the data set is stored in a database in which
neither the spatial indices (such as the popular R-tree) nor the
kNN-Join algorithms are available. Another limitation of the
existing approaches that are outside the relational database, is
the lack of support for query optimization, when additional
query conditions are specified. Consider the query:

Visualization tools such as 
PowerBI~\cite{powerbi}, Tableau~\cite{tableau}, QlikView~\cite{qlik}, and Zenvisage~\cite{zenvisagevldb} let users select one or more visualizations of their interest, and automatically show the related visualizations. For instance, Figure~\ref{fig:tableaudash} depicts a dashboard in Tableau where a market analyst selects the visualization of Boeing stock price to visualize other companies with similar stock trends over time. Similarly, Figure~\ref{fig:zenvisagedash} depicts a dashboard in Zenvisage, where a real estate analyst can either drag or drop the visualization of a specific state, or write a query in a table to find other states with similar housing price trends. 

In order to support such applications, it is crucial for a database query language to be able to {\em succinctly} express common comparative queries, and for query processing system to be able to efficiently evaluate such queries.
Unfortunately, standard SQL (SQL92) does not allow the concise expression of a number of conceptually
simple queries involving (potentially repeated) grouping and aggregation over the same groups. In order
to express such queries in SQL, one has to perform
additional joins, or to construct additional subqueries,
while a kind of sequential processing of the grouped
relation would be sufficient. The SQL versions of many
such queries show a high degree of redundancy. There
are two important consequences of such redundancy.
First, it is very difficult to write, understand, and
maintain such queries. Second, it is very difficult for
a query optimizer to identify efficient algorithms.







Visualization tools support expression or formula languages (e.g., Data Analysis Expressions (DAX) in PowerBI~\cite{powerbidax}, Level of Detail (LOD) expressions in Tableau~\cite{tableaulod}, ZQL in Zenvisage~\cite{zenvisagevldb}) that facilitate specification of comparison criteria using simple aggregates (e.g. \asum, \aavg, \amin, \amax),  and scalar functions. Internally, the queries are translated into one or more SQL queries for performing computations inside the databases, that helps avoid large data transfer delays, as well as serialization and deserialization overheads between the client and databases. In addition, it is also common for data analysts to directly issue custom SQL queries via connectors~\cite{customsql} supported in visualization tools, as well as using interactive data analytics IDEs such as SQL editors~\cite{sqleditor} and Jupyter notebooks~\cite{d2018aida,sqljupyter} for exploring visualizations. Unfortunately, the impedance mismatch between the operators in databases and the comparative analytical queries result in complex and inefficient SQL queries that hinder the performance of such queries, in some cases resulting in worse performance than their counterparts doing processing outside the databases. Therefore, in this work, our goal is to address this impedance mismatch for efficiently executing comparative queries inside the databases. We first give a few motivating examples, and describe the key limitations of existing SQL execution of comparative queries.

\eat{At the backend, visualization tools translate user interactions  into one or more SQL queries and issue them to relational database management systems (RDBMS) for execution. Unfortunately, the impedance mismatch between the operators in RDBMS and visualization queries result in complex and inefficient SQL queries that hinder the performance of such queries.
%(expressed in domain specific language)
At the backend, visualization tools translate user interactions  into one or more SQL queries and issue them to relational database management systems (RDBMS) for execution. Unfortunately, the impedance mismatch between the operators in RDBMS and visualization queries result in complex and inefficient SQL queries that hinder the performance of such queries.
An alternative is to run these queries outside the RDBMS in a middleware, unfortunately for large datasets such as approach incurs large overheads in terms of communication, and serialization and deserialization overheads between the processes.



We first give a few motivating examples, and then explain the limitations of SQL-based execution of comparative queries.
}


\eat{
	Data visualization is one of the primary mechanisms for 
	extracting and exploring insights from datasets. Visualization tools such as 
	PowerBI~\cite{powerbi}, Tableau~\cite{tableau}, QlickView~\cite{qlik}, and Zenvisage~\cite{zenvisagevldb}, powered by domain specific languages (e.g., PowerQuery~\cite{webb2014power},  VizQL~\cite{hanrahan2006vizql}, ZQL~\cite{zenvisagevldb},), support interactive interfaces to let users select one or more visualizations of their interest, and automatically find related visualizations. Such comparative queries facilitate rapid exploration by helping users fast-forward to their desired insights without requiring manual comparison. For example, Figure~\ref{fig:tableaudash} depicts a dashboard in Tableau where a market analyst selects the visualization of Boeing to find visualizations for other companies with similar stock trends over time. Similarly, Figure~\ref{fig:zenvisagedash} depicts a dashboard in Zenvisage, where a real estate analyst can either drag or drop the visualization of a state, or write a query in Zenvisage's domain specific langauge (ZQL~\cite{zenvisagevldb}) to find other states with similar housing price trends.
	
	The user interactions and domain-specific queries are translated by visualization tools into one or more SQL queries and are issued against relational database management systems (RDBMS) for execution. 
	Unfortunately, the existing operators in RDBMS are extremely limited when it comes to expressing comparative queries. This impedance mismatch between the specification of comparative queries in visualization systems and the operators supported in RDBMS often results in complex and inefficient SQL queries, that hinders the overall performance, especially as the dataset size or the number of visualizations increases. Thus, in this work, our goal is to address this impedance mismatch by extending RDBMS for more easily and efficiently supporting comparative queries. Before we discuss our core ideas, we characterize the main limitations of the existing SQL execution of comparative queries.
}

%Each visualization corresponds to subset of tuples in relation, and given one or more subsets of tuples as a reference, a comparative query returns $K$ other related subsets from the same relation, using a comparison function (e.g., Euclidean distance, mean absolute deviation) that measures the \emph{aggregated difference}  between the tuples of two subsets on some attribute (e.g., profits,

%In order to avoid the large data transfer latency, and serialization and deserialization overheads between the processes, visualization tools typically tr
%Even, the processing of these queries outside the RDBMS does not scale well due to the large data transfer latency, and serialization and deserialization overheads between the processes. 

\eat{
	One of the most common operations in data visualization is comparison~\cite{polaris,powerbi, ding2019quickinsights,lee2019you, seedb-tr,zenvisagevldb,wongsuphasawat2017voyager,macke2018adaptive}.
	Many visualization tools support mechanism to issue such queries ...
	However, very often they push it down to SQL queries to ...
	
	Comparative queries, involving comparison and filtering among subsets of data, are dominant in many visual and data exploration systems. . Real estate analysts compare house pricing trends using one or most cities as reference 
	(Figure~\ref{fig:zenvisagedash} depicts a Zenvisage~\cite{zenvisagevldb} query). Similarly, biologists search for and visualize genes based on comparing expressions patterns with a set of well-known genes~\cite{tatusov2000cog}. 
	In all these examples, given one or more subsets of tuples in a relation as a reference, a comparative query returns $K$ other related subsets from the same relation, 
	using a comparison function (e.g., Euclidean distance, mean absolute deviation) that measures the \emph{aggregated difference}  between the tuples of two subsets on some attribute (e.g., profits, price). 
}

% We classify these examples as \emph{comparative queries}, comprising a large class of data exploration use-cases. 
%Specifically, given a few interesting subsets of data as a reference and a user-specified comparison criteria, which in many cases are simple combinations of scalar and aggregation  functions (e.g., sum of differences, euclidean distance, mean absolute deviation), the goal of a comparative query is to return $K$ other (interesting) subsets of data as results.




\eat{
\begin{figure*}	
	\vspace{-15pt}
	\hspace{-0.2cm}
	\begin{subfigure}{0.38\textwidth}
		\vspace{-5pt}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/tableau-snapshot.pdf}}}}
		\caption{\smallcaption{Stock similarity search		in Tableau~\cite{tableau}}}
		\label{fig:tableaudash}
	\end{subfigure}
	\hspace{0.2cm}
	\begin{subfigure}{.38\textwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/zenvisage-snapshot.pdf}}}}	
		\caption{\smallcaption{Searching states with comparable housing price trends in Zenvisage~\cite{zenvisagevldb} }}
		\label{fig:zenvisagedash}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.20\textwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/motivation5.pdf}}}}
		\caption{\smallcaption{Mechanics of a \\ Comparative Query \fixlater{fix}}}
		\label{fig:comaparemechanics}
	\end{subfigure}
	\vspace{-10pt}
	\caption{ \smallcaption{a and b depict comparative queries in Tableau and Zenvisage, and c depicts the mechanics of a comparative query.} }
	\label{fig:motiv}	
		\vspace{-5pt}
\end{figure*} 
}



\eat{
	\begin{figure}
		\centerline {
			\hbox{\resizebox{.60\columnwidth}{!}{\includegraphics{./figs/sqlquery.pdf}}}}
		\caption{\smallcaption{An illustration of a comparative query. Using a few reference subset of tuples (shaded green), that  depict interesting patterns (as shown via trendline visualizations on the right), the goal is to find $k$ other subset of tuples (shaded gray) using an aggregated distance function. }}
		\label{fig:relationmotiv}
		\vspace{-10pt}
	\end{figure}
}

\eat{
	\begin{figure}
		\centerline {
			\hbox{\resizebox{.60\columnwidth}{!}{\includegraphics{./figs/motivation4.pdf}}}}
		\caption{\smallcaption{An illustration of a comparative query. Using a few reference subset of tuples (shaded green), that  depict interesting patterns (as shown via trendline visualizations on the right), the goal is to find $k$ other subset of tuples (shaded gray) using an aggregated distance function. }}
		\label{fig:relationmotiv}
		\vspace{-10pt}
	\end{figure}
}

\eat{
	e.g., visual queries in data exploration systems, similarity queries in multimedia databases, time-series analysis, genetics, text matching, information retrieval, and scientific databases.
	
	\emph{Given a few interesting subsets of data as a reference and a user-specified comparison criteria, which in many cases are simple aggregate functions, comparative queries return $K$ other subsets of data as results.} For example, in health analytics, physicians often explore and visualize the  physiological signals (e.g., diastolic readings) of the patients with similar to that of a reference patient. Market analysts search for products with profits to that of worst performing products. Researchers often search for and visualizes genes based on comparing expressions patterns with a set of well-known genes. 
	
	
	The increasing importance of comparative queries warrants an efficient support in the relational database management system (RDBMS), for \emph{comparing and filtering subsets of tuples} processing and filtering data as early in the pipeline as possible. As such, it has recently gained the attention of the research community. However, most of the available solutions for supporting
	comparative queries are in the middleware scenario \cite{tableau, seedb-tr, zenvisagevldb,voyager}, sitting outside the core of RDMBS. Hence,
	comparative queries are not treated as first-class query type, losing the
	advantages of integrating comparison-based operations with other relational operations. On the other hand, the typical approach in middleware-based systems is to pull the data out of the databases for performing comparison and filtering in the application. Clearly, because of the data transfer latency as well as serialization and deserialization overheads, these system do not scale well over large datasets stored at remote locations.
	
	% Since these analyses are usually performed with a human in the loop, a low-latency query response is highly advantageous. 
	
	
	Fundamental support of comparative queries is lacking in RDBMS mainly because relational algebra has no notion for 	\emph{comparison among subsets}. Therefore, supporting comparative queries in RDBMS's as a first-class query type is a significant research challenge. 
	In this paper, we present \system (short for 
	\textbf{C}omparative Queries \textbf{O}ptimization in \textbf{R}elation \textbf{D}atabases), a system for providing a seamless support and
	integration of comparative queries with the existing SQL query facility in
	relational database systems.
}

\eat{
	%The ubiquity of comparative queries across all applications warrants an efficient support for \emph{comparing and filtering subsets of tuples} in the relational database management system (RDBMS).
	Despite the ubiquity of comparative queries in data exploration, relational database management systems (RDBMS) are extremely slow in performing \emph{comparison among subsets of tuples}, often taking orders of magnitude more time compared to their counterparts running outside the core of RDBMS. Unfortunately, as the size of dataset increases, running these queries outside the core of RDBMS does not scale well owing to large data transfer, and serialization and deserialization overheads between the processes.
	
	
	

	To address these issues, we extend a commercial DBMS, \db, for efficiently supporting comparative queries inside the database engine. In particular, we show that by making query optimizer aware of the notion of comparison and introducing an efficient physical operator, we can achieve orders of magnitude better performance compared to the performance of physical plans generated by existing relational engines. Before we discuss our core ideas, we characterize the main limitations of the existing query execution strategy.
}

\eat{
	\begin{figure*}
		\begin{subfigure}{\columnwidth}
			\centerline {
				\hbox{\resizebox{.50\columnwidth}{!}{\includegraphics{./figs/motivation1.pdf}}}}
			\caption{\smallcaption{Illustrating a comparative query. Subset }}
			\label{fig:relationmotiv}
		\end{subfigure}
		\hspace{0.5cm}
		\begin{subfigure}{\columnwidth}
			\centering
			\hbox{\resizebox{0.7\columnwidth}{!}{\includegraphics{./figs/queryplan.pdf}}}
			\caption{\smallcaption{A query plan produced by optimizers for comparative queries}}
			\label{fig:queryplanmotiv}
		\end{subfigure}
		\vspace{-10pt}
		\caption{Comparative Queries}
		\vspace{-5pt}
		\label{fig:productresults}	
	\end{figure*}
}

\stitle{Motivating examples.} A market analyst, exploring sales trends of visualizations, notices that the sales of product ``Inspiron'' have been rising and falling irregularly within a specific range for the past $5$ years. To understand better, she is interested in finding $10$ additional products with similar behaviour, using different criteria. 

\textbf{Query 1.} \textit{Visualize $10$ products where the sum of the squared differences in sales per week with that of product Inspiron is minimum.}  To issue this query, the market analyst selects the visualization of Inspiron, and writes the comparison criteria using high-level expressions supported by visualization tools. In addition to the sum of squared differences, other aggregated distance measures such as $L_p$ norms can also be used for comparing trends.

%Since the sales behaviour of two products may not exactly align by week, another option is to
\textbf{Query 2.}  \emph{Visualize $10$ products that have similar distribution of sales values to that of Inspiron}. Two distributions are similar if they have small differences between any two sales values, and can be computed using Max-Min or Hausdorff distance~\cite{hung2004similarity}.


%Comparison criteria such as Euclidean distance and Max-Min can be easily expressed as aggregations (e.g., \asum, \aavg, \amin, \amax) of scalar expressions (differences, squared differences), hence these queries are typically translated  into SQL queries for in-database processing. Unfortunately, the SQL execution suffers with the following limitations.

\eat{
	\stitle{Limitations of SQL execution} Both these queries are typically translated  into SQL queries for in-database processing. Unfortunately, the SQL execution suffers with the following limitations.
}

As illustrated in Figure~\ref{fig:comaparemechanics}, both these queries are examples of a comparative query, where given a group of tuples for a reference product (shaded in green), the goal is to compare them with tuples corresponding to other products, and visualize $10$ products with similar trends or distributions. 

\stitle{Limitations of SQL execution.}  Since the queries involve simple aggregates and scalar expressions, they can be translated into one or more SQL queries for execution. Unfortunately, the SQL execution suffers with the following limitations.

\stitle{P1. Complex SQL query.} Figure~\ref{fig:querymotiv} depicts the SQL query,  similar to ones generated by visualization tools such as Tableau, with Figure~\ref{fig:planmotiv} depicting a simplified version of the query plan generated by \db for this SQL  query. 
As can be seen, the query is quite complex, requiring three sub-queries, two joins, and two scans. At a high level, the query first creates an intermediate relation via a self-join between the tuples of product Inspiron and the rest of the products (highlighted in red). Next, a sequence of scalar operations and aggregations  are performed on the intermediate relation to compute the similarity (, i.e., sum of squared differences) score of each product with Inspiron. Finally, a filter followed by a join operation output the tuples of $10$ products with minimum scores. 

To the best of our knowledge, both Figure~\ref{fig:querymotiv} and Figure~\ref{fig:planmotiv} are representative of how other relational databases will also express and execute queries such as query $1$, and are arguably the most optimal way of executing query $1$ with standard relational operators such as scan, join, aggregation, filters, and window analytics function such as rank.
While it is difficult for data analysts to directly write such a query, even when it is automatically generated, the complexity results in  long execution times because of the missed optimization opportunities that we discuss next.

%An easier specification mechanism could be to express the semantics of a comparative query more clearly, by  specifying 1) the reference and the candidate set of products to be compared, 2) an expression (e.g., Euclidean distance) for comparing the tuples of candidate products with reference product a score, and 3) a filtering criteria for selecting products based on their scores. Unfortunately, it is difficult to do so easily using existing SQL clauses.

\eat{
An ideal approach is to perform a join between product 'Inspiron' and each product separately using a process similar to Merge join.

sort tuples for each product on column "week", and independently  compare them with product ``Inspiron" using a process similar to Merge join.
}

\stitle{P2. Large number of tuple comparisons.} 
The self-join essentially performs all-pairs comparisons between the tuples of the reference group and the rest of the groups, with the overall number of comparisons proportional to product of the size of the reference group and  the size of all other groups. For example, if there are $100$ products, each consisting of $10^3$ tuples, the self-join in query $1$ performs a total of $10^3 \times 99 \times 10^3$ tuple comparisons. However, in many cases, all pairs comparisons can be avoided by performing \emph{groupwise comparisons, i.e., comparing each group independently with the reference group}. For example, for query 1, sorting tuples of each product on week and then comparing them independently reduces the number of comparisons by a factor of $10^3$ (i.e, the the size of each group), and is extremely parallelizable --- both leading to massive speed-up in performance. Unfortunately, the self-joins in relational databases do not support the notion of \emph{group-wise comparisons},  thereby missing potential optimizations.


\eat{
Suppose there are $100$ products, each consisting of $1000$ tuples. For Query 1, the self-join compares each tuple of product 'Inspiron' with every tuple of the rest of the products, performing a total of $99 \times 1000 \times 1000$ tuple comparisons. On the other hand, if we consider the tuples corresponding to each product independently, and sort them on week, we can follow a process similar to Merge join for comparing them with tuples of product ``Inspiron" in an ordered manner. This approach performs only $99 \times 1000$ comparisons, a factor $1000$ (i.e., the size of groups) less than the SQL execution. While comparing each product independently requires partitioning and sorting tuples, the speed-up due to much fewer tuple comparisons and parallel processing is typically large. Unfortunately, the relational databases miss the notion of \emph{group-wise comparison} here, resorting to the traditional way of performing self-join with many more tuple comparisons. 
}

%While there is a small overhead incurred in partitioning for grouping tuples for each product, the speed-up due to fewer tuple comparisons and parallel comparison is much more. Unfortunately, the relational databases miss the semantics of ``comparison among subset of tuples'' (e.g., one subset for each product)'' involved in these queries, thereby resorting to traditional way of performing self-join with many more tuple comparisons.


\stitle{P3. Large intermediate data.} 
The self-join results in generation of large intermediate data, i.e., one tuple for each pair of matched tuples between the reference group and other groups, which can be avoided without affecting the end results. For instance, for query 2, the self-join results in  $99 \times 10^6$ tuples since every tuple in  product 'Inspiron' is matched with every tuple of other products. The intermediate tuples are further materialized by subsequent operations (e.g., sort, aggregates) resulting in a substantial overhead. However, many comparison criteria, e.g., $L_p$ norms, involve simple aggregates (\aavg, \asum, \amin, \amax) and scalar operations such as differences, and thus comparison results can be computed efficiently in an incremental fashion (much like simple aggregates), without generating or materializing  intermediate tuples. 


\eat{
	\stitle{Problem 3. Large intermediate size.} The existing approach creates new tuples by joining all pairs of tuples between subsets that are compared. For example, if the number of 
	tuples for each product is $100$ and the number of products is $50$, the size of the intermediate table is $50.100^2$ times the original size of the relation. More specifically, the size of the intermediate relation is proportional to the number of tuples that are compared.
	The cost of performing a join to generate such large intermediate relations and performing subsequent operations (e.g., aggregation) that often require materialization (e.g, for sorting) is substantial. 
}

\stitle{P4. Comparison criteria agnostic.} Relational databases typically do not optimize for join and aggregation operations based on the scalar or aggregate  expressions that are computed on their output, missing key potential optimizations that can further reduce the number of tuple comparisons and runtimes of comparative queries. For example, consider a simple query where we want to find the \amax difference in the sales of two products.  Here, comparing only the tuples with smallest and largest values of sales for each product is sufficient. Unfortunately, the existing SQL execution performs a cross join, computing differences between all pairs of tuples from the  products, followed by an aggregation to find the \amax \xspace difference.

\stitle{P5. Missed inter-operator optimizations.} Finally, a comparative query can occur as a sub-query within a larger SQL query, with arbitrary relational expression such as joins as its input, and other operators consuming its output.  In those cases, we would ideally like the query optimizer to find a plan that is optimal for the entire query. Unfortunately, given the complexity of a comparative query, we observe that query optimizers are unable to apply even standard optimizations. Moreover, in certain cases such as PK-FK join, and aggregate queries, push-down and pull-up transformations can be applied to generate more efficient plans.


%pushed down below operators, or other operators such as filters and aggregates can be pushed down below a comparative quer
%and output the relation over which a comparative query can be expressed can be any arbitrary relational expression, involving multiple joins





%Because of the complex combination of multiple logical operator as depicted in the above query plan, the notion of comparison between subset of tuples is not straightforward to dissect. Moreover, existing optimizers analyze the properties (e.g., sorting, grouping, selectivity) on a per operator basis to select various logical optimizations such as below join push-down and predicate push-down. Unfortunately, we observe that the optimizers are unable to apply such optimizations for the entire sub-tree of logical operators.


\begin{figure}	
	\hspace{-0.2cm}
	\begin{subfigure}{0.55\columnwidth}
		\vspace{-8pt}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/sqlquery2.pdf}}}}
		
		\caption{\smallcaption{ SQL Query for Query 1} \fixlater{Fix}}
		\label{fig:querymotiv}
	\end{subfigure}
	\hspace{-0.6cm}
	\begin{subfigure}{.50\columnwidth}
		\centerline {
			\hbox{\resizebox{\columnwidth}{!}{\includegraphics{./figs/queryplan2.pdf}}}}
		\caption{\smallcaption{Query Plan for Query 1}}
		\label{fig:planmotiv}
	\end{subfigure}
	\vspace{-8pt}
	\caption{ \smallcaption{ The SQL Query and the query plan for Q1 that finds 10 products where the average minimum difference of sales to that of product 'Inspiron' is the smallest)} }
	\vspace{-5pt}
	\label{fig:productresults}	
	\vspace{-15pt}
\end{figure} 

\eat{
	
	\stitle{Motivating Example.} Anna, an infrastructure support analyst, notices unexpected changes in the cpu usage for $2$ machines, $M_1$ and $M_2$, over the past week as depicted in Figure~\ref{fig:relationmotiv}. For troubleshooting, she wants to understand whether there are additional machines with similar cpu usage profiles. The most commonly used metrics for comparing trends are $L_p$ norms such as Euclidean distance or sum of differences. If trends do not align point-wise over time, another option is to use \emph{min-max} aggregation, to find machines where maximum cpu usage differences with those of $M1$ or $M2$ between any two time point is minimum, or search for ones where the average difference in cpu across all points is minimum. Nevertheless, all these comparison functions are examples of aggregated distance functions, involving simple aggregations (e.g., $sum, avg, min, max$) over functions of differences. We list the three potential queries  using these comparison functions below.
	
	\emph{$Q1$. Visualize 10 machines that have smallest sum of differences in the cpu usage trends over hours with respect to those of $M_1$ and $M_2$.
	} 
	
	\emph{$Q2:$ Visualize $10$ machines whose maximum differences in CPU usages with those of $M1$ and $M2$ at any point during the week were smallest.}
	
	\emph{$Q3:$ Visualize $10$ machines whose average differences in the CPU usage with those of $M1$ and $M2$ across all points were smallest.}
	
	There are multiple ways to issue the above queries. The simplest option is to generate a large collection of visualizations, one for each machine and manually step through them to find the ones that have similar behaviour. Unfortunately, the process of manual examination is not scalable to $10$s of $1000$s of machines. Therefore, a better option is to either directly write a SQL query or use visual analytic tools that support high level language for expressing comparison among visualizations and automatically transform them to SQL queries. (e.g., Tableau's Level of Detail Expression, PowerBI's PowerQuery, Zenvisage, SeeDB).
	
	\stitle{ Existing query execution strategy.} 
	%While these queries differ in their comparison function, they all involve comparison between tuples across pairs of subsets of tuples. 
	Figure~\ref{fig:queryplanmotiv} depicts a simplified version of the query plan generated by RDBMS for executing SQL versions of above queries, and consists of five steps: (i) a filter to select $2$ subsets of tuples  (one each for $M_1$ and $M_2$), where a tuple records the CPU usage at a specific hour, (ii) a join between the tuples of the entire relation and reference subsets, generating an intermediate relation, (iii) a sequence of scalar operations and aggregations  to compute the aggregated distance ($score$) for every other machine, (iv) a filter to select the names of  $10$ machines with minimum scores, and finally (v) another join to select and output the subset of rows correspond to top $10$ machines. There are four  key problems with this execution strategy. 
	
	
	
	
	\eat{
		\begin{figure}
			\centerline {
				\hbox{\resizebox{.83\columnwidth}{!}{\includegraphics{./figs/queryplan.pdf}}}}
			\vspace{-10.5pt}
			\caption{\smallcaption{An example of a query plan produced by existing query optimizers for comparative queries in the motivating example.}}
			\label{fig:queryplanmotiv}
			\vspace{-10.5pt}
		\end{figure}
	}
	
	\eat{
		\begin{figure*}
			\centerline {
				\hbox{\resizebox{\textwidth}{!}{\includegraphics{./figs/diag1.pdf}}}}
			\vspace{-10.5pt}
			\caption{\smallcaption{Impact of the segment size on segment-aggregates based pruning $Q_1$}}
			\label{fig:varysegmentq1}
			\vspace{-2.5pt}
		\end{figure*}
	}
	
	\eat{
		\begin{figure}
			\centerline {
				\hbox{\resizebox{0.55\columnwidth}{!}{\includegraphics{./figs/queryplan2.pdf}}}}
			\caption{\smallcaption{An example query plan produced by optimizers for comparative queries}}
			\label{fig:queryplanmotiv}
			\vspace{-15.5pt}
		\end{figure}
	}
	
	\stitle{(1) Complex with redundant scan and join.} As depicted in the above query plan, expressing comparison between groups (or subsets) of tuples requires complex and redundant combination of multiple operations such as scans and joins. The is primarily because there is not direct mechanism for comparing groups (or subsets) of tuples in relational algebra, and it is extremely hard for an optimizer to dissect the notion of group-wise comparison abstracted across several operators in this plan. Moreover, there are no physical operators that support efficient algorithms for such operations. Finally, it is extremely hard to write, understand, and maintain such queries.
	
	
	\stitle{(2) Large intermediate size.} The existing approach creates new tuples by joining all pairs of tuples from subsets that are compared. For the above example involving two reference subsets and considering there are at least $100$ tuples for each machine, we see that the size of intermediate table for $Q_1$ is $2x$ more than the initial size, and for queries $Q_2$ and $Q_3$, the size is prohibitively large --- $100X$ the original size. Clearly, the cost of generating such large intermediate relations and performing subsequent operations (e.g., aggregation) on them is substantial. 
	
	
	\stitle{(3) Comparison agnostic.}  Comparison among subsets is typically done using aggregated distance functions as listed earlier, involving aggregation and scalar functions already supported in SQL. However, the existing execution approach is agnostic of  these functions, missing potential optimizations. As an extreme example, for finding maximum difference between two subsets, it is sufficient to to look at the differences among the tuples with maximum and minimum values. Unfortunately, the existing approach computes all differences between all pairs of tuples across the subsets, only to take the maximum; thereby wasting most of the effort.
	
	\stitle{(4) Missed inter-operator optimizations.} The optimzers leverage interesting properties to decide efficient plans that share grouping and sorting operations across operators. However, it is difficult to reason about such properties for a sub-graph of operators together. Similarly, it is difficult to apply logical optimizations such as join push-down and predicate push-down over the entire sub-graph.
	
}

\stitle{Our approach.} Our goal is to address the above limitations by reducing the complexity of query specification, and facilitating efficient processing of comparative queries. To do so,  we introduce both logical and physical extensions to relational databases, as described below.

\stitle{C1. Comparison as a first class construct (Section~\ref{sec:compareoverview})}. We introduce a new logical operation, \optr ($\Phi$), as a first class construct within the relational databases, and formalize its semantics that help capture a large class of frequently used comparative queries.  While \optr does not give additional expressive power to the relational algebra, it
reduces the complexity of specifying comparative queries and facilitates 
optimizations that are otherwise missed by the 
optimizer and the execution engine. We also propose extensions to SQL syntax
that allows intuitive and more concise specification of comparative queries.
%While it is also possible to extend the optimizer with algebraic transformation rules to translate comparative sub-queries expressed using standard SQL operators to $\Phi$.

%While \optr does not add to the expressivity of relational algebra,  it helps introduce the notion of subset comparison in the optimizer, making it easier to represent and reason about optimizations, as well as more effectively inter-operate with other relational operators.

\stitle{C2. Efficient processing via new physical operator (Section~\ref{sec:phyop})}. One option to execute \optr operation is to use user-defined functions (UDFs). However, UDFs have limited interoperability with other operators, and are less amenable to logical optimizations. We, therefore, introduce a new physical operator, $\Phi_P$, for the logical operator $\Phi$, that ensures  efficient execution of comparative queries. $\Phi_P$ exploits the semantics of \optr operation to partition and compare tuples in a manner that significantly reduces the number of tuple comparisons as well as the size of intermediate data.  In addition, $\Phi_P$ incorporates a number of physical optimizations that help avoid out many tuple comparisons for a large class of frequently used comparison functions without computing the exact results of groups.

\eat{
	For instance, for the example 1, $\Phi_P$ minimizes tuple comparisons and intermediate data by partitioning the input relation and performing comparison independently and in parallel for each product. In addition, $\Phi_P$ applies several physical optimizations that help in identifying the top $K$ products without computing the exact score. At a high-level, $\Phi_P$ can prune low scoring products without performing tuple-level comparisons by only comparing a few coarse-grained aggregates of partitions, that are faster to compute. Among the partitions that are not pruned, $\Phi_P$ further prioritizes tuple comparisons in an order that leads to faster convergence of the top $K$ partitions.
}
%For example, $\Phi_P$ summarizes sales of each product using coarse-grained aggregates that help prune out low scoring product without performing their tuple-level comparisons. $\Phi_P$ further prioritizes products that are most likely to be in top K and performs tuple comparison in an order that minimize wastage of tuple comparisons. 

\stitle{C3. Optimizer integration and logical optimizations (Section~\ref{sec:optint})}. 
We integrate \optr within the optimizer that enables automatic translation from logical ($\Phi$)  to physical ($\Phi_p$) operator using cost-based optimization.  We further extend the optimizer with algebraic transformation rules that allow logical optimizations when \optr occurs as a sub-query in a larger SQL query. 

% of queries where \optr occurs as a sub-component in a larger query. via reordering of \optr to minimize the overall query processing time of queries where \optr occurs as a sub-component in a larger query. 
\stitle{C4. Extensions (Section~\ref{sec:extensions}).}  
We  discuss four key extensions that build on the core ideas of \optr, including using multiple groups as references for comparison, supporting query-by-sketch systems~\cite{visual2, timesearcher,zenvisagevldb,lee2019you} where a sketch of the desired trend can be used as reference for finding similar groups, supporting user-defined functions (UDF), and handling missing values.


\stitle{C5. Implementation and evaluation (Section~\ref{sec:exp}).}  We have prototyped our techniques in \db engine, including both the logical and physical operators. We perform a thorough performance comparison of the extended \db with that of the unmodified \db on both real world and synthetic datasets. We also varied the characteristics of comparative queries to test the effectiveness and scalability of physical and logical optimizations. Overall, our experiments demonstrate that introducing \optr results in an improvement ranging from $3$$\times$ to $60$$\times$.

In  the rest of the paper, we describe each of the above contributions in detail.

%In summary, while \optr does not give additional expressive power to the relational algebra, it makes comparative queries much easier to write, and allows efficient processing via logical and physical optimizations that are difficult to apply with existing operators. In  rest of the paper, we describe each of the above contributions in detail.

\eat{
\stitle{Outline.} 
The rest of the paper is organized as follows. We first introduce the logical \optr ($\Phi$) operator  along with SQL extensions, and explain the semantics of comparative queries (Section 2). Next, we introduce a physical operator ($\Phi_p$) along with optimizations for efficient processing of \optr (Section 3). We then describe how we integrate $\Phi$ with the optimizer, discussing the cost modeling and logical  optimizations (Section 4). We  discuss three key extensions that build on core ideas of \optr from the earlier sections (Section 5). We present a thorough evaluation of \optr, comparing a number of variants of $\Phi$ with comparative queries executed using unmodified \db, as well as with a middleware-based approach (Section 6). Lastly, we  discuss the similarity and differences of \optr and proposed extensions with related work from databases and visualization area (Section 7). 
}

\vspace{-5pt}


\eat{
	We face such queries in the context of many database applications such as time-series analysis, genetics, text matching, information retrieval, and scientific databases. For example, in health analytics, physicians often explore and visualize the  physiological signals (e.g., diastolic readings) of the patients with similar to that of a reference patient. Market analysts search for products with profits to that of worst performing products. Researchers often search for and visualizes genes based on comparing expressions patterns with a set of well-known genes. Each of these examples involve a ``comparative query'' where the goal is to find a subset of datasets given a few subsets of data as reference, and comparison criteria as input and the goal 	
	(ii) subsets of data that are compared with the reference items, (iii) a comparison criteria, and (iv) number of items to be output. \cite{seeDb, VizRec, Zenvisage}. 
	We face such queries in the context of many database applications such as time-series analysis, recommendations systems, genetics, text matching, information retrieval, and scientific databases. In order to describe the challenges with existing approaches, we first describe a few illustrating examples.  Additional examples may be
	found in textbooks [DD92], business-related articles
	[KS95], and benchmarks [Cou95]. 
}


\eat{
	A data analysis workflow typically consists of two parts: \emph{exploration} followed by \emph{search}.  Exploration helps in getting the users familiarized with the dataset, primarily through visualizations that helps users see and understand hidden patterns in the datasets. This is followed by search,  which is more directed and user-driven, where the goal is to discover more interesting visualizations based on their comparison with visualizations of known items. For example, students making academic plans refer to friends; patients refer to acquaintances with similar conditions, physicians mention past cases seen in their practice.
	However, when working with large datasets, searching for visualizations that show interesting variations and similarities with known visualization is non-trivial: the analyst either manually compare  the patterns or trends among visualizations or issue complex queries in domain specific language  or SQL that take substantially long time to execute, both hampering the process of data exploration.
	
	conceptually more complex than necessary.
	
	
	In this paper, we tackle the problem of optimizing comparative analysis in relational databases. Comparative queries constitute a large class of data exploration queries, involving comparison among one or more subsets of data based on certain criteria (e..g., differences, similarity). To illustrate the challenges with existing approaches, we illustrate a few examples from real world domains.
	
	\vspace{2pt}
	\textsc{Example 1. Health Analytics}. 
	Physicians often explore data from similar patients to select the best treatment for a given patient. As a first step, the physician first retrieve and visualize the profile physiological signals of the patient. The analysts immediately noticed that while the weight of the patient was in the normal range, he had increasingly high diastolic readings for the last 5 days. To develop a health intervention plan for resolving the alerts of the patient, the analysts reviewed the activity summary of patients with similar changes in physiological behavior. Physician searches and visualizes 10 patients with similar behavior in their diastolic reading. Physician reviews the readings of these retrieved patients and poses additional queries to check medication that resolved their conditions.
	
	
	\vspace{2pt}
	\textsc{Example 2. Market Analytics}.    Recommender systems apply knowledge discovery techniques to the problem of making personalized recommendations for information, products or services during a live interaction. Given a few input items (liked by the user over the last few days), the goal  is to recommend top k other items that would be liked by the same user. An item $i$ has a higher chance of belonging to top-k if the users who liked input  items in the past items also liked the item $i$.
	
	\vspace{2pt}
	\textsc{Example 3. Market Analytics}.
	Max / Min example.
	
	
	Each of these examples is  a comparative query consisting of (i) subsets of data belonging to the reference items, (ii) subsets of data that are compared with the reference items, (iii) a comparison criteria, and (iv) number of items to be output. \cite{seeDb, VizRec, Zenvisage}. 
	We face such queries in the context of many database applications such as time-series analysis, recommendations systems, genetics, text matching, information retrieval, and scientific databases. In order to describe the challenges with existing approaches, we first describe a few illustrating examples.  Additional examples may be
	found in textbooks [DD92], business-related articles
	[KS95], and benchmarks [Cou95]. 
	\\
	
	\tar{Build a case for deviation.}
	
	\tar{Build a case for cross join.}
	
	\tar{Build a case for max min.}
	
	
	\subsection{Limitations of Current Techniques}
	Current state of-the-art visualization systems and tools fall into three categories. They (i) do not perform any comparison, or (ii) comparison outside of the database in a middleware, or (iii) comparison inside the databases via complex SQL queries.  
	
	
	\textsc{A. Manual exploration}. Specifying a comparative query is cumbersome, as result the de facto approach is generate all visualizes and manually compare them with the anchor visualizations. This approach is not scalable and becomes tedious and error-prone as the size of the dataset increases.
	
	
	\textsc{B. Middleware support}.  In state-of-the-art visual analytics tools, e.g., Tableau, QlikView, SAP Lumira, etc. domain specific languages help users specify the comparative queries. Even with these domain specific languages, users have to do many redundant operations. Recently, standalone visual data exploration systems have been proposed that provide a query languages that make it easier to specify comparative queries. However, all these tools issue  issue queries that retrieve the necessary data from the database, followed by performing comparison to identify subsets of data to be visualized. There are several disadvantages with such an approach. 
	First, when reading data from high volume data sources, result sets often contain millions of rows. This leads to very high bandwidth consumption between the tool and relational databases and consequently longer waiting times for the users. This becomes a serious bottleneck when the data is stored in a remote location. 
	
	Second, we found that time take for serialization and deserialization of data records before performing the comparison is non trivial, which increases proportionally with the size of the data.
	Missed optimization opportunities. Finally, middle-ware based data comparison also often causes both the database and middleware to perform redundant computations, across the database and middleware. 
	
	Similarly, middleware needs to perform redundant computations.
	
	\vspace{2pt}
	
	\textsc{C. In-Database Computation.} A potentially faster alternative is to rewrite the SQL queries to push the comparison and filtering operations within the databases. The reduced data volumes can mitigate high network bandwidth requirements and lead to shorter waiting times for the users of the visualization system. 
	All examples are cumbersome to express using standard SQL.
	
	Unfortunately, standard SQL does not allow the concise expression of a number of comparative  queries involving (potentially repeated) comparison among subset of rows in the same relation. Consequently, the rewritten SQL queries are often very complex, often taking more time than the middleware-based approach. To illustrate,  Table X depicts the rewritten SQL query for example 2 discussed above.
	
	There are four  key problems with the current query plans generated for comparative queries. 
	
	
	\stitle{1. Redundant Scan and Join.}  In order to express such queries in SQL, one has to perform multiple joins, or  construct additional subqueries, while a kind of simple comparison-based processing of the grouped relation would be sufficient. The SQL versions of many such queries show a high degree of redundancy. There are two important consequences of such redundancy. First, it is very difficult to write, understand, and maintain such queries. Second, it is very difficult for a query optimizer to identify efficient algorithms for such queries, as we illustrate later in the paper.
	
	
	\stitle{2. Large Intermediate Data Generation.} A consequence of using joins is  large intermediate relation for The cost of generating large relations and performing subsequent operations (e.g., aggregation) on the large intermediate relation is often substantial. For example, in query x. 
	
	
	\noindent
	\stitle{3. Computation Agnostic.}  The existing strategy for comparing two subsets is agnostic of  the comparison metric. For example, if we want to find max difference in values of a particular column for two relations, existing query plans tend to do full join, followed by computation of the difference. 
	As Section 1
	discussed, this approach fully materializes and aggregates all tuples, and then fully materializes and sorts all groups. Since only
	top-k groups are requested, much of the effort is simply wasted.
	
	\noindent
	\stitle{4. Missed Reuse and Sharing Opportunities.}
	Like the middleware-based 
	
	
	
	\subsection{Our Approach and Contributions}
	
	As noted above, there is  a communication and complexity tradeoff. In this paper, our goal is to develop techniques for optimizing comparative queries within the database.
	
	A number of papers and systems
	propose extensions of standard SQL in order to more
	easily express and optimize complex queries [CR96, KS95,
	RBVG96, Syb94]. Each of these proposals makes the
	argument that with an extended syntax, complex queries
	are easier to write and easier to optimize. We did not
	consider an extended syntax here, because (a) we wanted
	our work to apply to present-day systems, (b) we wanted to
	see how much optimization potential there was for queries
	without utilizing the hints inherent in a special syntax,
	and (c) we did not want to restrict the class of queries
	we considered in any way. Our techniques apply to all
	relational queries, including those expressed in a special
	syntax. 
	
	In this paper we define an extension to SQL syntax
	that allows the succinct representation of various comparison queries.
	We also propose a new relational algebra operation
	that concisely represents comparison among subset of rows. 
	We show how the operator can be implemented using
	efficient algorithms. We then show how queries can be
	translated from our SQL extension into our extended
	relational algebra. Our queries are significantly shorter
	and simpler than their standard SQL counterparts,
	and are much more easily optimized.  While our operator
	does not give additional expressive power to the relational algebra,
	it allows an important subset of queries
	to be succinctly expressed and efficiently evaluated.
	We implemented a version of our extended SQL
	language on top of a commercial relational database
	system. We compare the performance of the extended
	system on examples in our exended language to that
	of the underlying commercial system on standard SQL
	representations of the same examples. Our experimental results demonstrate orders of magnitude improvements in performance. We argue that extending SQL
	in a fashion similar to ours is essential in order for
	the query optimizer to be able to identify and utilize
	efficient evaluation techniques.
}
}
